On the achievable diversity-multiplexing tradeoff in interference channels

We analyze two-user single-antenna fading interference channels with perfect receive channel state information (CSI) and no transmit CSI. For the case of very strong interference, we prove that decoding interference while treating the intended signal as noise, subtracting the result out, and then decoding the desired signal, a process known as "stripping", achieves the diversity-multiplexing tradeoff (DMT) outer bound derived in Akuiyibo and Leveque, Int. Zurich Seminar on Commun., 2008. The proof is constructive in the sense that it provides corresponding code design criteria for DMT optimality. For general interference levels, we compute the DMT of a fixed-power-split Han and Kobayashi type superposition coding scheme, provide design criteria for the corresponding superposition codes, and find that this scheme is DMT-optimal for certain multiplexing rates.

==> Makefile <==
# LaTeX Makefile for use with the CTGTeX workflow
# generated Wed, 19, Nov, 2008 16:32:31UTC

# project directory: /Users/akcabac/ctguser/cakcaba/ISIT09
# project name, i.e., name of master latex file without ".tex" extension
PROJ = isit09

# additional (.tex) files that LaTeX depends on, i.e.macro files
AUX = cakcaba-macros.tex 

# graphics files used by \includegraphics
FIGS = 

# set to nonempty value to enable BibTeX
USEBIBTEX = 1

# is .bbl file in CVS? Leave blank if no, set to 1 if .bbl in CVS.
# If set to 1, bibtex won't be run (in order not to clobber the .bbl file).
BBLINCVS = 

# include master makefile
include $(CTGTEXDIR)/scripts/Pdflatex.mk

